Near-Optimal Regret for Policy Optimization in Contextual MDPs with General Offline Function Approximation

We introduce \texttt{OPO-CMDP}, the first policy optimization algorithm for stochastic Contextual Markov Decision Process (CMDPs) under general offline function approximation. Our approach achieves a high probability regret bound of $\widetilde{O}(H^4\sqrt{T|S||A|\log(|\mathcal{F}||\mathcal{P}|)}),$ where $S$ and $A$ denote the state and action spaces, $H$ the horizon length, $T$ the number of episodes, and $\mathcal{F}, \mathcal{P}$ the finite function classes used to approximate the losses and dynamics, respectively. This is the first regret bound with optimal dependence on $|S|$ and $|A|$, directly improving the current state-of-the-art (Qian, Hu, and Simchi-Levi, 2024). These results demonstrate that optimistic policy optimization provides a natural, computationally superior and theoretically near-optimal path for solving CMDPs.

==> mathdefs.tex <==
%%Requeiried packages and preliminary definitions, needed by the options
% \RequirePackage{mathtools}
% % \RequirePackage{thmtools}
  \RequirePackage{amsfonts}
 \RequirePackage{dsfont}
% \RequirePackage{delimset}
% \usepackage{amsmath}
 \usepackage{amssymb}


%%Body of the package, most of the declarations appear here.

\newcommand{\R}{\mathbb{R}} %reals
\newcommand{\N}{\mathbb{N}} % naturals
%\newcommand{\Reg}{\text{E.Regret}}
\newcommand{\Regrv}{\mathcal{R}}

\newcommand{\Reals}{\mathbb{R}} %reals
\newcommand{\Naturals}{\mathbb{N}} % naturals
\newcommand{\Var}{\mathbb{V}}%Variance
\newcommand{\E}{\mathbb{E}} % expectation
\newcommand{\Prob}{\mathbb{P}} % probability

\newcommand{\I}{\mathbb{I}} %indicator
\newcommand{\B}{\mathcal{B}} %Bernoulli rv
\newcommand{\V}{\mathbb{V}} % variance






\newcommand{\innProd}[2][*]{\brk[a]#1{#2}}
\newcommand{\ceil}[2][*]{\delim\lceil\rceil#1{#2}}
\newcommand{\floor}[2][*]{\delim\lfloor\rfloor#1{#2}}
\newcommand{\indEvent}[2][*]{\I_{\brk[c]#1{#2}}}
% \newcommand{\indEvent}[2][*]{\mathbb{1}{\brk[c]#1{#2}}}
\newcommand{\indFunc}[2][\infty]{\I_{\brk[s]{#2,#1}}}
\newcommand{\indFuncAt}[3][\infty]{\indFunc[#1]{#2}\brk*{#3}}
\newcommand{\tr}[2][*]{\mathrm{Tr}\brk*{#2}}
\newcommand{\overbar}[1]{\mkern 2mu\overline{\mkern-2mu#1\mkern-2mu}\mkern 2mu}
\newcommand{\tran}{^{\mkern-1.5mu\mathsf{T}}}


% Standard Math Notations
\newcommand{\Oof}[2][*]{O\brk#1{#2}}
\newcommand{\OtildeOf}[2][*]{\smash{\widetilde{O}}\brk#1{#2}}

\newcommand{\poly}{\mathrm{poly}}


\newcommand{\Tau}{\mathcal{T}}



% Probability
\newcommand{\gaussDist}[2]{\mathcal{N}\brk0{#1, #2}}

% Math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}



% General
\def\noi{\noindent}

\newcommand{\ifrac}[2]{#1/#2}

\newcommand{\rootT}{\ensuremath{\smash{\sqrt{T}}}\xspace}

==> thmdefs.tex <==
%%Requeiried packages and preliminary definitions, needed by the options
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{thmtools}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREM STYLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%% standard

% \declaretheoremstyle[
% 	    spaceabove=\topsep, 
% 	    spacebelow=\topsep, 
% 	    bodyfont=\normalfont\itshape,
%     ]{theorem}

% \declaretheorem[style=theorem,name=Theorem]{theorem}

% \declaretheoremstyle[
% 	    spaceabove=\topsep, 
% 	    spacebelow=\topsep, 
% 	    bodyfont=\normalfont,
%     ]{definition}
    
%%%%%% JMLR-style

\setlength{\topsep}{\medskipamount}

\declaretheoremstyle[
	    spaceabove=\topsep, 
	    spacebelow=\topsep, 
	    headfont=\normalfont\bfseries,
	    bodyfont=\normalfont\itshape,
	    notefont=\normalfont\bfseries,
	    notebraces={(}{)},
	    postheadspace=0.33em, 
	    headpunct={.},
	   % postfoothook=\noindent\ignorespaces
    ]{theorem}
% \declaretheorem[style=theorem,numberwithin=section]{theorem}
\declaretheorem[style=theorem]{theorem}

\declaretheoremstyle[
	    spaceabove=\topsep, 
	    spacebelow=\topsep, 
	    headfont=\normalfont\bfseries,
	    bodyfont=\normalfont,
	    notefont=\normalfont\bfseries,
	    notebraces={(}{)},
	    postheadspace=0.33em, 
	    headpunct={.},
	   % postfoothook=\noindent\ignorespaces
    ]{definition}

\let\proof\undefined
\declaretheoremstyle[
        spaceabove=\topsep, 
        spacebelow=\topsep, 
        headfont=\normalfont\bfseries,
        bodyfont=\normalfont,
        notefont=\normalfont\bfseries,
        % notebraces={(}{)},
        notebraces={}{},
        postheadspace=0.33em, 
        qed=$\blacksquare$, 
        headpunct={.},
        % postfoothook=\noindent\ignorespaces
    ]{proofstyle}
\declaretheorem[style=proofstyle,numbered=no,name=Proof]{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		
\declaretheorem[style=theorem,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=theorem,sibling=theorem,name=Corollary]{corollary}
\declaretheorem[style=theorem,sibling=theorem,name=Claim]{claim}
\declaretheorem[style=theorem,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=theorem,sibling=theorem,name=Fact]{fact}
\declaretheorem[style=theorem,sibling=theorem,name=Observation]{observation}
\declaretheorem[style=theorem,sibling=theorem,name=Conjecture]{conjecture}

\declaretheorem[style=theorem,numbered=no,name=Theorem]{theorem*}
\declaretheorem[style=theorem,numbered=no,name=Lemma]{lemma*}
\declaretheorem[style=theorem,numbered=no,name=Corollary]{corollary*}
\declaretheorem[style=theorem,numbered=no,name=Proposition]{proposition*}
\declaretheorem[style=theorem,numbered=no,name=Claim]{claim*}
\declaretheorem[style=theorem,numbered=no,name=Fact]{fact*}
\declaretheorem[style=theorem,numbered=no,name=Observation]{observation*}
\declaretheorem[style=theorem,numbered=no,name=Conjecture]{conjecture*}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,sibling=theorem,name=Remark]{remark}
\declaretheorem[style=definition,sibling=theorem,name=Example]{example}
\declaretheorem[style=definition,sibling=theorem,name=Question]{question}

\declaretheorem[style=definition,numbered=no,name=Definition]{definition*}
\declaretheorem[style=definition,numbered=no,name=Remark]{remark*}
\declaretheorem[style=definition,numbered=no,name=Example]{example*}
\declaretheorem[style=definition,numbered=no,name=Question]{question*}

\declaretheorem[style=theorem,sibling=theorem,name=Assumption]{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
